Unsupervised ensemble-based phenotyping helps enhance the discoverability of genes related to heart morphology

Recent genome-wide association studies (GWAS) have been successful in identifying associations between genetic variants and simple cardiac parameters derived from cardiac magnetic resonance (CMR) images. However, the emergence of big databases including genetic data linked to CMR, facilitates investigation of more nuanced patterns of shape variability. Here, we propose a new framework for gene discovery entitled Unsupervised Phenotype Ensembles (UPE). UPE builds a redundant yet highly expressive representation by pooling a set of phenotypes learned in an unsupervised manner, using deep learning models trained with different hyperparameters. These phenotypes are then analyzed via (GWAS), retaining only highly confident and stable associations across the ensemble. We apply our approach to the UK Biobank database to extract left-ventricular (LV) geometric features from image-derived three-dimensional meshes. We demonstrate that our approach greatly improves the discoverability of genes influencing LV shape, identifying 11 loci with study-wide significance and 8 with suggestive significance. We argue that our approach would enable more extensive discovery of gene associations with image-derived phenotypes for other organs or image modalities.

==> figs_per_locus.tex <==
\begin{figure*}[ht!]
\centering
\includegraphics[width=\textwidth]{figs/supplementary/figs_per_locus/chr6_78.png}
\caption{Triad of plots for locus PLN.}
\label{fig:chr6_78}
\end{figure*}

\begin{figure*}[ht!]
\centering
\includegraphics[width=\textwidth]{figs/supplementary/figs_per_locus/chr2_108.png}
\caption{Triad of plots for locus TTN.}
\label{fig:chr2_108}
\end{figure*}

\begin{figure*}[ht!]
\centering
\includegraphics[width=\textwidth]{figs/supplementary/figs_per_locus/chr12_69.png}
\caption{Triad of plots for locus TBX5.}
\label{fig:chr12_69}
\end{figure*}

\begin{figure*}[ht!]
\centering
\includegraphics[width=\textwidth]{figs/supplementary/figs_per_locus/chr17_27.png}
\caption{Triad of plots for locus GOSR2.}
\label{fig:chr17_27}
\end{figure*}

\begin{figure*}[ht!]
\centering
\includegraphics[width=\textwidth]{figs/supplementary/figs_per_locus/chr5_103.png}
\caption{Triad of plots for locus NKX2.5.}
\label{fig:chr5_103}
\end{figure*}

\begin{figure*}[ht!]
\centering
\includegraphics[width=\textwidth]{figs/supplementary/figs_per_locus/chr13_37.png}
\caption{Triad of plots for locus LMO7.}
\label{fig:chr13_37}
\end{figure*}


\begin{figure*}[ht!]
\centering
\includegraphics[width=\textwidth]{figs/supplementary/figs_per_locus/chr10_69.png}
\caption{Triad of plots for locus RBM20.}
\label{fig:chr10_69}
\end{figure*}

\begin{figure*}[ht!]
\centering
\includegraphics[width=\textwidth]{figs/supplementary/figs_per_locus/chr8_18.png}
\caption{Triad of plots for locus CNOT7.}
\label{fig:chr8_18}
\end{figure*}

\begin{figure*}[ht!]
\centering
\includegraphics[width=\textwidth]{figs/supplementary/figs_per_locus/chr10_20.png}
\caption{Triad of plots for locus WAC.}
\label{fig:chr10_20}
\end{figure*}

\begin{figure*}[ht!]
\centering
\includegraphics[width=\textwidth]{figs/supplementary/figs_per_locus/chr1_124.png}
\caption{Triad of plots for locus near gene LGALS8.}
\label{fig:chr1_124}
\end{figure*}

\begin{figure*}[ht!]
\centering
\includegraphics[width=\textwidth]{figs/supplementary/figs_per_locus/chr12_19.png}
\caption{Triad of plots for locus near gene CCDC91.}
\label{fig:chr12_19}
\end{figure*}

\begin{figure*}[ht!]
\centering
\includegraphics[width=\textwidth]{figs/supplementary/figs_per_locus/chr2_69.png}
\caption{Triad of plots for locus near gene EN1.}
\label{fig:chr2_69}
\end{figure*}

\begin{figure*}[ht!]
\centering
\includegraphics[width=\textwidth]{figs/supplementary/figs_per_locus/chr10_74.png}
\caption{Triad of plots for locus near gene BAG3.}
\label{fig:chr10_74}
\end{figure*}

\begin{figure*}[ht!]
\centering
\includegraphics[width=\textwidth]{figs/supplementary/figs_per_locus/chr11_32.png}
\caption{Triad of plots for locus near gene OR9Q1.}
\label{fig:chr11_32}
\end{figure*}

\begin{figure*}[ht!]
\centering
\includegraphics[width=\textwidth]{figs/supplementary/figs_per_locus/chr2_23.png}
\caption{Triad of plots for locus STRN.}
\label{fig:chr2_23}
\end{figure*}




==> tables/corr_with_cardiac_indices.tex <==
\begin{table*}[ht!]
\begin{center}
\begin{tabular}{lrrrr}
\toprule
{} &  LVEDV &  LVEDSph &    LVM &  LVMVR \\
\midrule
PLN    &  0.434 &    0.625 &  0.333 & -0.158 \\
GOSR2  & -0.335 &   -0.272 & -0.397 & -0.148 \\
TTN    &  0.889 &   -0.157 &  0.904 &  0.224 \\
TBX5   &  0.888 &    0.000 &  0.761 & -0.035 \\
NKX2.5 & -0.865 &   -0.372 & -0.790 &  0.002 \\
LMO7   &  0.927 &   -0.014 &  0.832 &  0.021 \\
RBM20  &  0.971 &    0.070 &  0.887 &  0.040 \\
CNOT7 & -0.900 &   -0.135 & -0.902 & -0.191 \\
WAC    &  0.888 &   -0.120 &  0.903 &  0.199 \\
LGALS8  &  0.672 &    0.227 &  0.605 & -0.061 \\
CCDC91 &  0.499 &    0.248 &  0.358 & -0.156 \\
EN1    & -0.041 &   -0.461 & -0.137 & -0.112 \\
BAG3   &  0.928 &    0.089 &  0.841 &  0.018 \\
OR9Q1  &  0.528 &    0.603 &  0.440 & -0.107 \\
STRN   & -0.165 &   -0.429 & -0.183 & -0.296 \\
\bottomrule
\end{tabular}
\caption{Spearman correlation between the best phenotypes per locus and four LV handcrafted indices.}
\end{center}
\label{table:corr_with_indices}
\end{table*}
